Towards Efficient Exact Synthesis for Linear Hybrid Systems

We study the problem of automatically computing the controllable region of a Linear Hybrid Automaton, with respect to a safety objective. We describe the techniques that are needed to effectively and efficiently implement a recently-proposed solution procedure, based on polyhedral abstractions of the state space. Supporting experimental results are presented, based on an implementation of the proposed techniques on top of the tool PHAVer.

==> eptcsdata.tex <==
\providecommand{\firstpage}{263}
\providecommand{\publicationstatus}{Giovanna D'Agostino, Salvatore La Torre (Eds.):\\
Proceedings of the Second International Symposium on\\ 
``Games, Automata, Logics and Formal Verification'' (GandALF 2011)\\
EPTCS 54, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.54.19}{10.4204/EPTCS.54.19}}
\pdfoutput=1

